Description of the CUDF Format

This document contains several related specifications, together they describe the document formats related to the solver competition which will be organized by Mancoosi. In particular, this document describes: - DUDF (Distribution Upgradeability Description Format), the document format to be used to submit upgrade problem instances from user machines to a (distribution-specific) database of upgrade problems; - CUDF (Common Upgradeability Description Format), the document format used to encode upgrade problems, abstracting over distribution-specific details. Solvers taking part in the competition will be fed with input in CUDF format.

==> debian-dudf.tex <==

\section{\sc Debian-DUDF}

In this section we describe the instantiation of DUDF to Debian, that is the
\textsc{Debian-DUDF} format.

\paragraph{Package status} The current local package status is always available
on disk in the file \linebreak \PATH{/var/lib/dpkg/status}, which is in RFC 822
format with one stanza for each package. Sending it as an extensional section
would do.

If the version uniqueness assumption \pageref{req:versionkey} is verified, the
section can be sent partially in intensional form, by projecting each package
stanza to the fields: \texttt{Package}, \texttt{Status}. Even when the
assumption is not verified, several other fields can be dropped, most notably
\texttt{Description} which account for most of the file total size.

Specific tools use extra information as part of their local package status view.
For example aptitude uses \PATH{/var/lib/aptitude/pkgstates}.

\paragraph{Package universe} The universe of all packages considered for an
upgrade problem is available on disk as the lists of packages known by APT. They
are stored under \PATH{/var/lib/apt/lists/} and match the filename pattern
\texttt{*\_Packages}. Such files are downloaded when the APT \texttt{update}
action is required and are a local cache of package indexes coming from the
Debian archive or its mirrors around the world.

For each repository listed in \PATH{/etc/apt/sources.list} there are several
package lists stored on disk, one for each section (e.g: main, contrib,
non-free) of that archive which is listed in \PATH{sources.list} (plus other
auxiliary files which are not relevant for the moment). Only lists corresponding
to repositories which were active at the time of the last update are kept on
disk; lists for repositories which have been removed from \PATH{sources.list}
are removed upon the next update run.

Sending all the lists as an extensional section will provide a suitable package
universe for a submission. However the required size for the transfer can be
prohibitive.

For a given set of ``well-known'' repositories an alternative is to send as an
intension just the md5sums of the corresponding lists.  As the lists are byte to
byte local copies of the remote repositories one can rely on them to retrieve a
posteriori the whole lists from some historical mirror. The package lists are
equal among different (synchronized) mirrors; this property is granted by
the apt-secure machinery, as differences would invalidate the Release file
signed with the GPG keys of the master Debian archive. To avoid having to look
up server side among all possible md5sums, it seems wise to send the date of
last modification of the file lists on disk together with the architecture
specification, to be used as a rough guide about where the exact md5sums has to
be found.\ZACK{actually the architecture is also needed to know how to handle
dependencies which are conditional on the current architecture, not only as an
optimization. This needs to be stated explicitly somewhere else}

In case we want to send also the mirror URLs (for the sake of some server side
control?), URLs can be retrieved quite easily as the file names are trivial
transliterations of the origin URLs, e.g.:
{\small\verb+security.debian.org_dists_testing_updates_main_binary-i386_Packages+}

Note that for a submission to be useful, all potentially involved packages in
the universe need to be known. As such a submission of just some lists will be
useless (unless of course the ignored lists are known to not be taking part in
the upgrade). When only some of the lists are known to be encodable
intensionally, the remaining lists should be sent extensionally.\ZACK{this
raises the observation that the submission clients should know what archives are
available server side to expand intensional references. As a protocol to
discover this sounds overkilling, we probably should decide from the beginning
which package repositories will be supported intensionally and which will not.}

\paragraph{Requested action} A trivial textual encoding of user requested action
\pageref{sec:action} is in order. Easy, but TODO.

\paragraph{Desiderata}

This section is way too open to describe precisely a Debian-based format.
However some legacy Debian files can be already considered as implicit sources
of non-functional desiderata and should be better sent as part of a submission.
We list them here briefly:

\begin{itemize}

 \item \PATH{/etc/apt/preferences} lists the user preferences with distribution
  she wants her packages coming from. The same information, in a much more
  parseable way can be extracted from the output of \texttt{apt-policy};

\end{itemize}

\paragraph{(Resulting) package status}

TODO

\subsubsection{Measures}

Some approximate, rule of thumb, numbers to have an idea of the involved sizes.
Numbers have been snapshot-ed on 18/04/2008, on a i386 Debian Sid machine. The
numbers per se are basically meaningless since they are affected by many
factors, they are there just to have an idea of the order of magnitude of a
potential submission. Also, they have been measured with \texttt{du}, as such
the sizes are disk blocks which overestimate the real byte count.

\PATH{/etc/apt/sources.list} contains all sections of both Debian Sid and Debian
Testing, a well-known repository for multimedia applications which can't be
distributed by Debian, and the usual security repositories.

\begin{center}
\begin{tabular}{l|r|r|p{4cm}}
 \hline
 \textbf{section} & \textbf{plain} & \textbf{compressed} (gzip)
  & \textbf{notes} \\
 \hline
 \emph{package status} & & & \\
 \hspace{1em} \PATH{\small /var/lib/dpkg/status} & 2.5 Mb & 748 Kb
  & {\small 160 Kb / 24 Kb with trimmed stanzas} \\
 \hline
 \emph{package universe} & & & \\
 \hspace{1em} \PATH{\small /var/lib/apt/lists/*\_Packages} & 48 Mb & 14 Mb
  & {\small reduces to 14 Kb for just sending the list md5sums together with
  \PATH{sources.list}} \\
 \hline
 \emph{requested action} & & & \\
 \hline
 \emph{resulting package status} & & & \\
 \hline
\end{tabular}
\end{center}


